AttributionBench: How Hard is Automatic Attribution Evaluation?

Modern generative search engines enhance the reliability of large language model (LLM) responses by providing cited evidence. However, evaluating the answer's attribution, i.e., whether every claim within the generated responses is fully supported by its cited evidence, remains an open problem. This verification, traditionally dependent on costly human evaluation, underscores the urgent need for automatic attribution evaluation methods. To bridge the gap in the absence of standardized benchmarks for these methods, we present AttributionBench, a comprehensive benchmark compiled from various existing attribution datasets. Our extensive experiments on AttributionBench reveal the challenges of automatic attribution evaluation, even for state-of-the-art LLMs. Specifically, our findings show that even a fine-tuned GPT-3.5 only achieves around 80% macro-F1 under a binary classification formulation. A detailed analysis of more than 300 error cases indicates that a majority of failures stem from the model's inability to process nuanced information, and the discrepancy between the information the model has access to and that human annotators do.

==> figures/error_categories.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{.45\textwidth} % 占据页面宽度的 45%
        \includegraphics[width=\textwidth]{figures/error_categories.pdf} % 插入 PDF 的第一页
        \caption{Error types.}
        \label{fig:error_cases}
    \end{minipage}
    % 可以在此处添加其他内容或另一个 minipage
\end{figure}

==> latex/methodology.tex <==
% \section{Task Formulation}
% \label{sec:task_formulation}

% % \subsection{Task Formulation}
% The input of the attribution evaluation task involves these following components: (1) a natural language query $Q$, (2) a generated response $R$ consisting of several claims, and a reference set $E=\{e_1, e_2, ..., e_n\}$ from an attributed LLM. Every generated response $R$ consists of several claims $c_i$, each of which represents a single sentence in the response $R$. Each claim $c_i$ has a bunch of corresponded references $e_i = \{e_{i1}, e_{i2}, ..., e_{ij}\}$.

% For the label space, some previous works define it as a three-way classification (``Support'', ``Partially Support'', and ``No Support'') or involve fine-grained error classes (``Attributable'', ``Contradictory'', ``Extrapolatory'').
% For simplicity and compatibility, here we define the attribution evaluation task as a binary-classification task: $Labels = \{"Attributable", "Not Attributable"\}$.
% For the evaluation metrics, we use accuracy and macro average F1 score, to measure the model's overall performance on both positive and negative labels.
% The claim-level evaluator model is defined as a classifier $f(\cdot)$. It's supposed to take $\langle , c_i, (R), concat\{e_i\}\rangle$ as the input, where $concat\{e_i\}$ is the concatenation of all the corresponded references $e_{ij}$ of $c_i$. Note that the question $Q$ and the response $R$ are optional to occur in the input, since the basic goal of this task is to evaluate whether the references can support the claim or not. Other information fields can be seen as additional information that helps the model evaluate the attribution.

==> tables/different_input_fields.tex <==
\begin{table*}[h]
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{cc|cccc|c|ccc|c}

\toprule[1pt]
\multirow{1}{*}{\textbf{Model}} & \multirow{1}{*}{\textbf{Input Fields}} & \multirow{1}{*}{\textbf{ExpertQA}} & \multirow{1}{*}{\textbf{Stanford-GenSearch}} & \multirow{1}{*}{\textbf{AttributedQA}} & \multirow{1}{*}{\textbf{LFQA}} & \multirow{1}{*}{\textbf{ID-Avg.}} & \multirow{1}{*}{\textbf{BEGIN}} & \multirow{1}{*}{\textbf{AttrEval-GenSearch}} & \multirow{1}{*}{\textbf{HAGRID}} & \multirow{1}{*}{\textbf{OOD-Avg.}} \\ \hline
\multirow{4}{*}{GPT-3.5-turbo-1106 (0-shot w/o CoT)} & \multirow{1}{*}{C+E} & \multirow{1}{*}{55.3} & \multirow{1}{*}{62.0} & \multirow{1}{*}{74.7} & \multirow{1}{*}{72.6} & \multirow{1}{*}{\textbf{66.2}} & \multirow{1}{*}{79.4} & \multirow{1}{*}{76.7} & \multirow{1}{*}{70.1} & \multirow{1}{*}{\textbf{75.4}} \\
 & \multirow{1}{*}{Q+C+E} & \multirow{1}{*}{57.2} & \multirow{1}{*}{59.0} & \multirow{1}{*}{73.9} & \multirow{1}{*}{64.2} & \multirow{1}{*}{63.6} & \multirow{1}{*}{78.7} & \multirow{1}{*}{77.1} & \multirow{1}{*}{64.0} & \multirow{1}{*}{73.3} \\
 & \multirow{1}{*}{C+E+R} & \multirow{1}{*}{42.8} & \multirow{1}{*}{44.9} & \multirow{1}{*}{58.1} & \multirow{1}{*}{39.3} & \multirow{1}{*}{46.3} & \multirow{1}{*}{72.4} & \multirow{1}{*}{58.9} & \multirow{1}{*}{40.2} & \multirow{1}{*}{57.2} \\
 & \multirow{1}{*}{Q+C+E+R} & \multirow{1}{*}{48.6} & \multirow{1}{*}{48.1} & \multirow{1}{*}{70.2} & \multirow{1}{*}{53.1} & \multirow{1}{*}{55.0} & \multirow{1}{*}{74.2} & \multirow{1}{*}{70.5} & \multirow{1}{*}{56.1} & \multirow{1}{*}{66.9} \\
 \midrule
 \multirow{4}{*}{Llama-2 (7B) (Fine-tuned)} & \multirow{1}{*}{C+E} & \multirow{1}{*}{60.5} & \multirow{1}{*}{80.2} & \multirow{1}{*}{79.9} & \multirow{1}{*}{85.6} & \multirow{1}{*}{76.6} & \multirow{1}{*}{84.1} & \multirow{1}{*}{83.3} & \multirow{1}{*}{73.0} & \multirow{1}{*}{80.1} \\
 & \multirow{1}{*}{Q+C+E} & \multirow{1}{*}{62.3} & \multirow{1}{*}{81.8} & \multirow{1}{*}{79.5} & \multirow{1}{*}{87.5} & \multirow{1}{*}{\textbf{77.8}} & \multirow{1}{*}{85.7} & \multirow{1}{*}{84.5} & \multirow{1}{*}{74.8} & \multirow{1}{*}{\textbf{81.7}} \\
 & \multirow{1}{*}{C+E+R} & \multirow{1}{*}{60.6} & \multirow{1}{*}{80.2} & \multirow{1}{*}{77.3} & \multirow{1}{*}{82.1} & \multirow{1}{*}{75.1} & \multirow{1}{*}{77.5} & \multirow{1}{*}{84.5} & \multirow{1}{*}{69.2} & \multirow{1}{*}{77.1} \\
 & \multirow{1}{*}{Q+C+E+R} & \multirow{1}{*}{60.6} & \multirow{1}{*}{80.8} & \multirow{1}{*}{82.5} & \multirow{1}{*}{84.5} & \multirow{1}{*}{77.1} & \multirow{1}{*}{83.0} & \multirow{1}{*}{84.5} & \multirow{1}{*}{72.8} & \multirow{1}{*}{80.1} \\
 
\bottomrule[1pt]
\end{tabular}
}
\caption{The performance (F1 score) with different input fields on each dataset. Q, C, E, R stands for question, claim, evidence, and response, respectively. ZS: zero-shot, FT: fine-tuned. Results shows that manipulating input fields doesn't bring a huge effect to the performance.}
\label{your-label}
\end{table*}

==> tables/different_instructions.tex <==
\begin{table*}[h]
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{cc|cccccccc}

\toprule[1pt]
\multirow{1}{*}{\textbf{Input Fields}} & \multirow{1}{*}{\textbf{Model}} & \multirow{1}{*}{\textbf{ExpertQA}} & \multirow{1}{*}{\textbf{Stanford-GS}} & \multirow{1}{*}{\textbf{HAGRID}} & \multirow{1}{*}{\textbf{AttributedQA}} & \multirow{1}{*}{\textbf{LFQA}} & \multirow{1}{*}{\textbf{BEGIN}} & \multirow{1}{*}{\textbf{AttrEval-GS}} & \multirow{1}{*}{\textbf{Overall}} \\ \hline
\multirow{3}{*}{Q + C + E} & \multirow{1}{*}{GPT-3.5-turbo-16k (ZS)} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} \\
 & \multirow{1}{*}{GPT-4-0613 (ZS)} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} \\
 & \multirow{1}{*}{Llama 2 (7B) (FT)} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} \\
 \hline
 \multirow{3}{*}{C + E} & \multirow{1}{*}{GPT-3.5-turbo-16k (ZS)} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} \\
 & \multirow{1}{*}{GPT-4-0613 (ZS)} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} \\
 & \multirow{1}{*}{Llama 2 (7B) (FT)} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} \\
 \hline
 \multirow{3}{*}{Q + C + E + R} & \multirow{1}{*}{GPT-3.5-turbo-16k (ZS)} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} \\
 & \multirow{1}{*}{GPT-4-0613 (ZS)} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} \\
 & \multirow{1}{*}{Llama 2 (7B) (FT)} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} & \multirow{1}{*}{-} \\
 
\bottomrule[1pt]
\end{tabular}
}
\caption{The performance (F1 score) with different input fields on each dataset. Q, C, E, R stands for question, claim, evidence, and response, respectively. ZS: zero-shot, FT: fine-tuned. Results shows that manipulating input fields doesn't bring a huge effect to the performance.}
\label{your-label}
\end{table*}
